Crossing The Gap: A Deep Dive into Zero-Shot Sim-to-Real Transfer for Dynamics

Zero-shot sim-to-real transfer of tasks with complex dynamics is a highly challenging and unsolved problem. A number of solutions have been proposed in recent years, but we have found that many works do not present a thorough evaluation in the real world, or underplay the significant engineering effort and task-specific fine tuning that is required to achieve the published results. In this paper, we dive deeper into the sim-to-real transfer challenge, investigate why this is such a difficult problem, and present objective evaluations of a number of transfer methods across a range of real-world tasks. Surprisingly, we found that a method which simply injects random forces into the simulation performs just as well as more complex methods, such as those which randomise the simulator's dynamics parameters, or adapt a policy online using recurrent network architectures.

==> reward_table.tex <==
\begin{table}[h]
\begin{tabular}{cc}
Env. & Reward  \\
 Reaching & $- \norm{d_{po}} - \sum_joints \mathbbm{1}_{lim} - \mathbbm{1}_{table} $\\
 Pushing &  \\
 Sliding & 
\end{tabular}
\end{table}
